AfroLID: A Neural Language Identification Tool for African Languages

Language identification (LID) is a crucial precursor for NLP, especially for mining web data. Problematically, most of the world's 7000+ languages today are not covered by LID technologies. We address this pressing issue for Africa by introducing AfroLID, a neural LID toolkit for $517$ African languages and varieties. AfroLID exploits a multi-domain web dataset manually curated from across 14 language families utilizing five orthographic systems. When evaluated on our blind Test set, AfroLID achieves 95.89 F_1-score. We also compare AfroLID to five existing LID tools that each cover a small number of African languages, finding it to outperform them on most languages. We further show the utility of AfroLID in the wild by testing it on the acutely under-served Twitter domain. Finally, we offer a number of controlled case studies and perform a linguistically-motivated error analysis that allow us to both showcase AfroLID's powerful capabilities and limitations.

==> tables/all_data.tex <==
\begin{table*}[h!]
\small
\begin{tabular}{ccccccccccc}
\textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} & \textbf{ISO-3} \\
aar      & bmo      & dua      & gud      & kdl      & lem      & mgh      & nhu      & rub      & tiv      & xtc      \\
aba      & bmv      & dug      & gur      & kdn      & lgg      & mgo      & nih      & run      & tke      & xuo      \\
abn      & bom      & dwr      & guw      & kea      & lgm      & mgq      & nim      & rwk      & tlj      & yal      \\
acd      & bov      & dyi      & gux      & ken      & lia      & mgr      & nin      & sag      & tll      & yam      \\
ach      & box      & dyu      & guz      & khy      & lik      & mgw      & niy      & saq      & tog      & yao      \\
ada      & bqc      & ebr      & gvl      & kia      & lin      & mif      & nka      & sba      & toh      & yat      \\
adh      & bqj      & ebu      & gwr      & kik      & lip      & mkl      & nko      & sbd      & toi      & yba      \\
adj      & bsc      & efi      & gya      & kin      & lmd      & mlg      & nla      & sbp      & tpm      & ybb      \\
afr      & bsp      & ego      & hag      & kiz      & lmp      & mlr      & nnb      & sbs      & tsc      & yom      \\
agq      & bss      & eka      & har      & kki      & lnl      & mmy      & nnh      & sby      & tsn      & yor      \\
aha      & bst      & eko      & hau      & kkj      & log      & mnf      & nnq      & sef      & tso      & yre      \\
ajg      & bud      & eto      & hay      & kln      & lom      & mnk      & nnw      & ses      & tsw      & zaj      \\
akp      & bum      & etu      & hbb      & klu      & loq      & moa      & nse      & sev      & ttj      & zdj      \\
alz      & bun      & etx      & heh      & kma      & lot      & mos      & nso      & sfw      & ttq      & zga      \\
amh      & bus      & ewe      & her      & kmb      & loz      & moy      & ntr      & sgw      & ttr      & ziw      \\
ann      & buy      & ewo      & hgm      & kmy      & lro      & moz      & nuj      & shi      & tui      & zne      \\
anu      & bwr      & fak      & hna      & knf      & lsm      & mpe      & nus      & shj      & tul      & zul      \\
anv      & bwu      & fat      & ibb      & kng      & lth      & mpg      & nwb      & shk      & tum      &                \\
asa      & bxk      & ffm      & ibo      & knk      & lto      & mqb      & nxd      & sid      & tuv      &                \\
asg      & byf      & fia      & idu      & kno      & lua      & msc      & nya      & sig      & tvu      &                \\
atg      & byv      & fip      & igb      & koo      & luc      & mur      & nyb      & sil      & twi      &                \\
ati      & bza      & flr      & ige      & koq      & lue      & muy      & nyd      & sna      & umb      &                \\
avn      & bzw      & fon      & igl      & kqn      & lug      & mwe      & nyf      & snf      & urh      &                \\
avu      & cce      & fub      & ijn      & kqp      & lun      & mwm      & nyk      & sng      & uth      &                \\
azo      & chw      & fue      & ikk      & kqs      & luo      & mwn      & nym      & snw      & vag      &                \\
bam      & cjk      & fuf      & ikw      & kqy      & lwg      & mws      & nyn      & som      & vai      &                \\
bav      & cko      & fuh      & iqw      & kri      & lwo      & myb      & nyo      & sop      & ven      &                \\
bba      & cme      & ful      & iri      & krs      & maf      & myk      & nyu      & sor      & vid      &                \\
bbj      & cop      & fuq      & ish      & krw      & mas      & myx      & nyy      & sot      & vif      &                \\
bbk      & cou      & fuv      & iso      & krx      & maw      & mzm      & nza      & soy      & vmk      &                \\
bci      & crs      & gaa      & iyx      & ksb      & mbu      & mzw      & nzi      & spp      & vmw      &                \\
bcn      & csk      & gax      & izr      & ksf      & mck      & naq      & odu      & ssw      & vun      &                \\
bcw      & cwe      & gaz      & izz      & ksp      & mcn      & naw      & ogo      & suk      & vut      &                \\
bcy      & daa      & gbo      & jgo      & ktj      & mcp      & nba      & oke      & sus      & wal      &                \\
bdh      & dag      & gbr      & jib      & ktu      & mcu      & nbl      & okr      & swa      & wbi      &                \\
bds      & dav      & gde      & jit      & kua      & mda      & ncu      & oku      & swc      & wec      &                \\
bem      & dga      & gid      & jmc      & kub      & mdm      & ndc      & orm      & swh      & wes      &                \\
beq      & dgd      & giz      & kab      & kuj      & mdy      & nde      & ozm      & swk      & wib      &                \\
ber      & dgi      & gjn      & kam      & kus      & men      & ndh      & pcm      & sxb      & wmw      &                \\
bex      & dhm      & gkn      & kbn      & kvj      & meq      & ndj      & pem      & taq      & wol      &                \\
bez      & dib      & gkp      & kbo      & kwn      & mer      & ndo      & pkb      & tcc      & won      &                \\
bfa      & did      & gmv      & kbp      & kyf      & mev      & ndv      & pko      & tcd      & xan      &                \\
bfd      & dig      & gna      & kby      & kyq      & mfe      & ndz      & pov      & ted      & xed      &                \\
bfo      & dik      & gnd      & kcg      & kzr      & mfg      & ngb      & poy      & tem      & xho      &                \\
bib      & dip      & gng      & kck      & lai      & mfh      & ngc      & rag      & teo      & xnz      &                \\
bim      & diu      & gof      & kdc      & laj      & mfi      & ngl      & rel      & tex      & xog      &                \\
bin      & dks      & gog      & kde      & lam      & mfk      & ngn      & rif      & tgw      & xon      &                \\
biv      & dnj      & gol      & kdh      & lap      & mfq      & ngo      & rim      & thk      & xpe      &                \\
bjv      & dow      & gqr      & kdi      & lee      & mfz      & ngp      & rnd      & thv      & xrb      &                \\
bky      & dsh      & gso      & kdj      & lef      & mgc      & nhr      & rng      & tir      & xsm      &               
\end{tabular}
\caption{ISO-3 codes for the all language varieties in our training data.}
\label{tab:allin_training}
\end{table*}

==> tables/diacritics_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
\multicolumn{1}{l}{\textbf{Name of diacritic}}         & \multicolumn{1}{l}{\textbf{Language}}    & \multicolumn{1}{l}{\textbf{Example}} &  \\
\toprule
grave accent                                           & Aghem                                    & Kə̀lestò                                          \\
acute accent                                           & Ebrié                                    & jisɛmánhɔn                                         \\
circumflex                                             & Akoose                                   & mesɔɔm-tê                                         \\
umlaut, trema or dieresis                              & Ewondo                                   & Yënë                                               \\
tilde                                                  & Bassa                                    & kɔ̃in                                              \\
cedilla                                                & tupuri                                   & waçaçge                                            \\
macron accent (a bar over the letter)                  & Nyakyusa-Ngode                           & popāpo                                             \\
bar under the letter                                   & nyimatli-tera                            & dlu̱dlarsi                                         \\
dot under the letter                                   & Babanki                                  & Ḅongong ḅongong                                    \\
caron/háček ("v") over the letter                      & Sepedi                                   & botša                                              \\
slashed o (o with stroke)                              & Anyuak                                   & Jwøk                                               \\
barred i                                               & Bafut                                    & bɨ                                                 \\
horn                                                   & Songhai de Gao - Koyraboro Senni Songhai & gʼi noo                                            \\
barred u                                               & Ghomálá'                                 & shwɔppfʉə                                          \\
breve under the letter                                 & pokomo                                   & Yud̯a                                              \\
accute accent over character and tilde under character & Sar    
\\
\toprule
\end{tabular}%
}
\caption{Example diacritics in our training data. \abdu{I think it's better to move this to appendix  due to space limitation.}}\label{tab:diacritics}
\end{table*}

==> tables/naija_senti_tweet_compare.tex <==
\begin{table*}[h!]
\begin{tabular}{llll}
Language & \textbf{BPE} & CHAR & WORD  \\
hau  & $89$ & $73.69$ & $73.24$ \\
ibo  & $46$ & $26.25$ & $55.48$ \\
pcm  & $56$ & $21.09$ & $61.94$ \\
yor  & $82$ & $75.92$ & $73.62$ \\
\end{tabular}
\caption{AfroLID performance on naijasenti validation datasets for $4$ languages covered in naijasenti corpus}
\label{tab:dev_naija_senti_tweet_results_comparison.}
\end{table*}

\begin{table*}[]
\begin{tabular}{llll}
Language & \textbf{BPE} & CHAR & WORD  \\
hau  & $74$ & $73.69$ & $73.24$ \\
ibo  & $42$ & $26.25$ & $55.48$ \\
pcm  & $65$ & $21.09$ & $61.94$ \\
yor  & $38$ & $75.92$ & $73.62$ \\
\end{tabular}
\caption{Frac performance on naijasenti validation datasets for $4$ languages covered in naijasenti corpus}
\label{tab:dev_naija_senti_tweet_results_comparison.}
\end{table*}

\begin{table*}[]
\begin{tabular}{llll}
Language & \textbf{BPE} & CHAR & WORD  \\
hau  & $92$ & $73.69$ & $73.24$ \\
ibo  & $100$ & $26.25$ & $55.48$ \\
pcm  & $98$ & $21.09$ & $61.94$ \\
yor  & $100$ & $75.92$ & $73.62$ \\
\end{tabular}
\caption{AfroLID performance on AfroLID validation datasets for $4$ languages covered in naijasenti corpus.}
\label{tab:dev_naija_senti_tweet_results_comparison}
\end{table*}

% \begin{table*}[]
% \begin{tabular}{llll}
% Language & \textbf{BPE} & CHAR & WORD  \\
% hau  & $89.56$ & $74.11$ & $71.18$ \\
% ibo  & $46.60$ & $24.62$ & $54.60$ \\
% pcm  & $61.63$ & $21.05$ & $71.02$ \\
% yor  & $82.86$ & $76.87$ & $74.94$ \\
% ALL*  & $73.36 $ & $55.08$ & $68.03 $ \\
% \end{tabular}
% \caption{}
% \label{tab:train_naija_senti_tweet_results_comparison}
% \end{table*}

==> typology.tex <==
\section{Genetic Classification}\label{sec:twitter}
Language classification otherwise referred to as genetic classification aims to group languages based on their similarity and distinctiveness. Genetically similar languages are classified into groups in such a way that languages with higher relationship are divided into similar classes while those with a lower degree of similarities are further divided into subclasses. Two genetically related languages can therefore be viewed as sisters of the same parent language. That is they are languages that evolved over time from an older parent language \cite{ludwig_2020}. 

Language classification differs from typological classification in that the former determines relationships based on genealogy or origin while the latter classifies languages based on grammatical features or types \cite{rainer_2020}. For instance, a typological classification will group tone languages together, or split languages based on their morphological structure into for example isolating or agglutinating languages. Despite this difference, languages that belong to the same genetic type often share similar typological information \cite{ludwig_2020}. For example, most Benue-Congo languages are tone languages. 
In the case of African languages where typological information is scarcely available, utilizing genetic classes may be a useful way to determine optimum ways for language processing. If the typological information of one language in a group is known, we may make a sensible assumption that other languages in that group may share similar features with minor variations. 

Based on this premise, we explore the genetic classification of $517$ African languages across $7$ language families also referred to as phyllum \cite{jeff_2020}. We use classification information as they exist on Ethnologue \cite{ethnologue}. We also provide some details about the languages in each family and some tree structures that show the relationships that exist between the languages within a family. Specifically, we provide tree structures for Afro-Asiatic, Austronesian, Creole, Indo-European, Khoe-Kwadi, Niger-Congo, and Nilo-Saharan for the $517$ languages in our dataset. Each family in our dataset contains $61$, $1$, $9$, $1$, $3$, $392$, and $62$ languages respectively. 
\subsection{Afro-Asiatic}
\subsection{Austronesian}
\subsection{Creole}
A creole language is one spoken initially only in situations of contact between speakers of two or more mutually unintelligible languages, and not as a language within an ethnic group \cite{sommer_2020}. Historically, creoles have evolved along trade routes or in colonized communities, particularly when several groups of people without a common lingua franca are forced to communicate in the presence of a dominant language. Creole languages therefore often include lexical items, and grammatical features from multiple contact languages. Although, one dominant language also referred to as the lexifier language contributes majority of the vocabulary. 

Creole languages are classified based on their geographical location and further grouped according to their main lexifier languages, their presumed origins, and the major contact languages.

\subsection{Indo-European}
\subsection{Khoe-Kwadi}
\subsection{Niger-Congo}
Niger-Congo also referred to as Niger-Kordofanian is the largest language family in Africa \cite{jeff_2020}, consisting of the highest number of languages and speakers. Niger-Congo languages spread across sub-Saharan Africa, with Benue-Congo, including Bantu languages dominating the southern part of the continent.  Niger-Congo languages are quite varied, especially with respect to their degree of morphological elaboration. This is also true of Benue-Congo, with some of its languages having an isolating morphological character and others showing extensive agglutinating morphology.

\subsection{Nilo-Saharan}
